Mochi: Fast \& Exact Collision Detection

Collision Detection (CD) has several applications across the domains such as robotics, visual graphics, and fluid mechanics. Finding exact collisions between the objects in the scene is quite computationally intensive. To quickly filter the object pairs that do not result in a collision, bounding boxes are built on the objects, indexed using a Bounding Volume Hierarchy(BVH), and tested for intersection before performing the expensive object-object intersection tests. In state-of-the-art CD libraries, accelerators such as GPUs are used to accelerate BVH traversal by building specialized data structures. The recent addition of ray tracing architecture to GPU hardware is designed to do the same but in the context of implementing a Ray Tracing algorithm to render a graphical scene in real-time. We present Mochi, a fast and exact collision detection engine that accelerates both the broad and narrow phases by taking advantage of the capabilities of Ray Tracing cores. We introduce multiple new reductions to perform generic CD to support three types of objects for CD: simple spherical particles, objects describable by mathematical equations, and complex objects composed of a triangle mesh. By implementing our reductions, Mochi achieves several orders of magnitude speedups on synthetic datasets and 5x-28x speedups on real-world triangle mesh datasets. We further evaluate our reductions thoroughly and provide several architectural insights on the ray tracing cores that are otherwise unknown due to their proprietorship.

==> 6discussion.tex <==



==> scrap.tex <==
% As the GPU compute ability increases, we have more tools and hardware support available at hand to boost CD performance \milind{Can cut this sentence. The first sentence flows nicely into the third sentence}. 

While we show we can use the RT-NNS reduction to solve a specialized case of CD where all the objects are spheres of equal radius, 

Not only does RT-NNS index more world space than necessary, but it also produces incorrect 

% \milind{It may be worth mentioning here that you could imagine just using the maximum radius, and then filtering out false positives, but the BVH will be very inefficient in this case -- you can cite the trueKNN paper for that point}
% If the scene has spheres of different radius, the previous reduction does not work because the reported intersections are at a distance of $2r_i$ but not $r_i+r_j$. 

% making things more complicated along two dimensions - shape and 
% transition-what case can we use existing reduction
% lets start simple
% So we need a bounding sphere of radius $2r$ to capture the collisions.
% The set of nodes that the ray touches during the traversal is the BVTT front.
% We will see in section\ref{} how remembering BVTT frame is not particularly helpful on RT cores.



This is possible on rtx because we found a way to formulate obj-obj intersections by building on ray-obj intersection.
we are performing obj-obj intersections by tracing the object(bounding volume) with the rays.
this remove indexing false worldly space as object space.

Mochi benefits from the RT cores, since it does not have to deal with the thread and memory divergence during the BVH traversal.

But the silver lining is that we do not have to put the triangles inside an AABB, since RT-cores natively support triangles as a geometric data type.


\begin{table*}
\centering
\begin{tabular}{ |c|c|c|c|l|l|l|l|l|l|l|l| } 
 \hline
 \multicolumn{4}{|c|}{\bfseries Dataset Info} & \multicolumn{3}{|c|}{\bfseries Mochi Refit} & \multicolumn{3}{|c|}{\bfseries Mochi Rebuild} & \multicolumn{2}{|c|}{\bfseries Oibvh}\\ \hline
 Name & Vertices & Triangles & Frames & \multicolumn{1}{|p{0.8cm}|}{Initial build time} & \multicolumn{1}{|p{1.1cm}|}{avg refit time per frame} & \multicolumn{1}{|p{1cm}|}{avg CD time per frame} & \multicolumn{1}{|p{0.8cm}|}{Initial build time} & \multicolumn{1}{|p{1.2cm}|}{avg rebuild time per frame} & \multicolumn{1}{|p{1cm}|}{avg CD time per frame} & \multicolumn{1}{|p{1.1cm}|}{avg build time per frame} & \multicolumn{1}{|p{1cm}|}{avg CD time per frame}\\ \hline
 Funnel & 9450 & 18484 & 500 & 1.93 & 0.69 & 0.20 & 2.16 & 1.79 & 0.14 & 2.26 & 1.82\\ 
 Flamenco & 25686 & 49218 & 706 & 2.78 & 1.63 & 0.36 & 2.16 & 2.87 & 0.24 & 6.62 & 6.92\\ 
 Cloth-ball & 46598 & 92230 & 94 & 4.23 & 2.31 & 0.59 & 2.72 & 4.07 & 0.35 & 7.71 & 1.85\\ 
 N-body & 73960 & 146480 & 76 & 4.61 & 4.00 & 7.83 & 3.04 & 5.45 & 0.39 & 63.55 & 9.68\\ 
 \hline
\end{tabular}
\caption{results on rtx2060, all times in milliseconds}
\label{table:1}
\end{table*}


plot showing variation in initial build time but no diff in refit time
not useful


% \begin{table}[h!]
% \begin{center}
% \begin{tabular}{ |c|c|c|c|c|c|c| } 
%  \hline
%   & 1st frame & refit & CD & 1st frame & rebuild & CD \\ \hline
%  Funnel & 1.41 & 0.26 & 0.16 & 1.42 & 0.99 & 0.10 \\ 
%  Cloth-ball & 38.50 & 0.48 & 0.92 & 48.01 & 1.6 & 0.13\\ 
%  N-body & 38.81 & 0.47 & 75.70 & 37.92 & 1.78 & 0.25\\ 
%  Drag-bun & 38.78 & 0.76 & 13.44 & 1.6 & 0.13 & \\ 
%  \hline
% \end{tabular}
%  \caption{results on TitanV}
% \end{center}
% \end{table}

\subsubsection*{Summary of Mochi principles} 
Trace the object by shooting rays along the edges of the object or its bounding box. 
At least one of the colliding objects is bound to report the intersection.




all the intersections that the rays report are the triangles that are colliding with this triangle.
edge rays of one of the traingles will intersect the other when two triangles collide 
if a triangle hits another triangle's face, a will report.
However, this approach fails to capture coplanar intersections, and thus an incomplete solution.



when two triangles are axis aligned, they dont intersect unless they overlap.


the number of triangles and vertices remain constant through out the frames.
% rebuild and refit
rt cores allow us refit the bvh.
refit api - what it does and how is it helpful.
existing techniques had to rely on refit since rebuild is very expensive but after enough nuber of frames the quality of bvh deters anyway.
It's not to say that rt cores rebuild is not expensive.
as the evaluation section \ref{} shows rebuild is x times slower than refit however, rebuild allows the rt cores to more efficiently trace the rays and traverse the bvh.

%if its an obb it would have been fine, but its aabb.
